Domain Adaptation with Cauchy-Schwarz Divergence

Domain adaptation aims to use training data from one or multiple source domains to learn a hypothesis that can be generalized to a different, but related, target domain. As such, having a reliable measure for evaluating the discrepancy of both marginal and conditional distributions is crucial. We introduce Cauchy-Schwarz (CS) divergence to the problem of unsupervised domain adaptation (UDA). The CS divergence offers a theoretically tighter generalization error bound than the popular Kullback-Leibler divergence. This holds for the general case of supervised learning, including multi-class classification and regression. Furthermore, we illustrate that the CS divergence enables a simple estimator on the discrepancy of both marginal and conditional distributions between source and target domains in the representation space, without requiring any distributional assumptions. We provide multiple examples to illustrate how the CS divergence can be conveniently used in both distance metric- or adversarial training-based UDA frameworks, resulting in compelling performance.

==> Figures/two_big_figures.tex <==
\begin{figure} 
%\hfill
\begin{minipage}[b]{.45\linewidth} 
%\centering 
     \begin{subfigure}[b]{0.7\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/compare_mnist.png}
         \caption{The ablation study of the \textbf{CS} and \textbf{CCS} components.}
         %  in MNIST to USPS task, comparing with MMD and joint distribution MMD (JPMMD)
         \label{Fig.abl-mnist}
     \end{subfigure}
     \begin{subfigure}[b]{0.7\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/compare_mnist_fdal.png}
         \caption{The ablation study of \textbf{f-DAL with CCS} divergence } 
         %  in MNIST to USPS task. CCS divergence improves the performance of f-DAL consistently.
         \label{fig:f-dal-ccs}
     \end{subfigure}
        \caption{Percent ($1$ indicates $100\%$) of correctly rejecting $H_0$ hypothesis with different values of $\mu$ and $\sigma^2$.}
        \label{fig:marginal_power}
\end{minipage}% 
%\hfill
\begin{minipage}[b]{.5\linewidth} 
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TSNE_25_no_adaptation.png}
         \caption{No adaptation}
         \label{fig:tsne-no-ad}
     \end{subfigure}
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TSNE_25_cs.png}
         \caption{CS divergence}
         \label{fig:tsne-cs}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TSNE_25_ccs.png}
        \caption{CCS divergence}
         \label{fig:tsne-ccs}
     \end{subfigure}
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TSNE_25_cs_ccs.png}
        \caption{CCS \& CS divergence}
         \label{fig:tsne-cs-ccs}
     \end{subfigure}
\caption{t-SNE visualization of feature trained without adaptation (\ref{fig:tsne-no-ad}), with CS divergence (\ref{fig:tsne-cs}, with CCS divergence (\ref{fig:tsne-ccs}), and with both CCS and CS divergences (\ref{fig:tsne-cs-ccs}).} 
\label{tab:fig:tsne-overall}
\end{minipage} 
\end{figure}


% \begin{figure} 
% \centering 
%      \begin{subfigure}[b]{0.3\textwidth}
%          \includegraphics[width=\textwidth]{Figures/compare_mnist.png}
%          \caption{The ablation study of the \textbf{CS} and \textbf{CCS} components in MNIST to USPS task, comparing with MMD and joint distribution MMD (JPMMD).}
%          \label{Fig.abl-mnist}
%      \end{subfigure}
%      \hspace{0.05\textwidth} % Add horizontal space
%      \begin{subfigure}[b]{0.3\textwidth}
%          \includegraphics[width=\textwidth]{Figures/compare_mnist_fdal.png}
%          \caption{The ablation study of \textbf{f-DAL with CCS} divergence in MNIST to USPS task. CCS divergence improves the performance of f-DAL consistently. }
%          \label{fig:f-dal-ccs}
%      \end{subfigure}
% \end{figure}



% \begin{figure} 
% %\hfill
% \centering 
%      \begin{subfigure}[b]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/TSNE_25_no_adaptation.png}
%          \caption{No adaptation}
%          \label{fig:tsne-no-ad}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/TSNE_25_cs.png}
%          \caption{CS divergence}
%          \label{fig:tsne-cs}
%      \end{subfigure}
%      %\hfill
%      \begin{subfigure}[b]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/TSNE_25_ccs.png}
%         \caption{CCS divergence}
%          \label{fig:tsne-ccs}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/TSNE_25_cs_ccs.png}
%         \caption{CCS \& CS divergence}
%          \label{fig:tsne-cs-ccs}
%      \end{subfigure}
%         \caption{t-SNE visualization of feature trained without adaptation (\ref{fig:tsne-no-ad}), with CS divergence (\ref{fig:tsne-cs}, with CCS divergence (\ref{fig:tsne-ccs}), and with both CCS and CS divergences (\ref{fig:tsne-cs-ccs}).}
%         \label{fig:tsne-overall}
% \end{figure}

==> Tables/office31.tex <==

% \begin{table*}[htbp]
% \centering
% \resizebox{0.7\textwidth}{!}{%
% \begin{tabular}{lccccccc}
% \toprule
% Method & A$\rightarrow$W & D$\rightarrow$W & W$\rightarrow$D & A$\rightarrow$D & D$\rightarrow$A & W$\rightarrow$A & Avg \\
% \midrule
% ResNet~\cite{he2016deep} & 68.4$\pm$0.2 & 96.7$\pm$0.1 & 99.3$\pm$0.1 & 68.9$\pm$0.2 & 62.5$\pm$0.3 & 60.7$\pm$0.3 & 76.1\\
% DANN~\cite{ganin2016domain} & 82.0$\pm$0.4 & 96.9$\pm$0.2 & 99.1$\pm$0.1 & 79.7$\pm$0.4 & 68.2$\pm$0.4 & 67.4$\pm$0.5 & 82.2 \\
% JAN~\cite{long2017deep} & 85.4$\pm$0.3 & 97.4$\pm$0.2 & 99.8$\pm$0.2 & 84.7$\pm$0.3 & 68.6$\pm$0.3 & 70.0$\pm$0.4 & 84.3 \\
% GTA~\cite{sankaranarayanan2018generate} & 89.5$\pm$0.5 & 97.9$\pm$0.3 & 99.8$\pm$0.4 & 87.7$\pm$0.5 & 72.8$\pm$0.3 & 71.4$\pm$0.4 & 86.5 \\
% MCD~\cite{saito2018maximum} & 88.6$\pm$0.2 & 98.5$\pm$0.1 & 100.0$\pm$.0 &92.2$\pm$0.2 & 69.5$\pm$0.1 & 69.7$\pm$0.3 & 86.5 \\
% KL~\cite{nguyen2021kl} & 87.9$\pm$0.4 & 99.0$\pm$0.2 & 100.0$\pm$0.0 & 85.6$\pm$0.6 & 70.1$\pm$1.1 & 69.3$\pm$0.7 & 85.3 \\
% CDAN~\cite{long2018conditional} & 94.1$\pm$0.1 & 98.6$\pm$0.1 & 100.0$\pm$.0 & 92.9$\pm$0.2 & 71.0$\pm$0.3 & 69.3$\pm$0.3 & 87.7 \\
% f-DAL~\cite{acuna2021f} & \textbf{95.4}$\pm$0.7 & \textbf{98.8}$\pm$0.1 & \textbf{100.0}$\pm$.0 & 93.8$\pm$0.4 & 74.9$\pm$1.5 & 74.2 $\pm$0.5 & 89.5 \\
% %f-DAL+Alignment~\cite{acuna2021f} & 93.4$\pm$0.4 & \textbf{99.0}$\pm$0.1 & \textbf{100.0}$\pm$.0 & 94.8$\pm$0.6 & 73.6$\pm$0.2 & 74.6$\pm$0.4 & 89.2 \\
% \midrule
% CS-adv (Ours) & 95.1$\pm$0.6 & \textbf{98.8}$\pm$0.1 &	99.7$\pm$0.1 & \textbf{94.0}$\pm$0.5 &	\textbf{76.2}$\pm$0.3 & \textbf{76.4}$\pm$0.4 &	\textbf{90.0} \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Comparative results (Accuracy \%) of different methods on \textbf{Office-31} dataset.}
% \label{tab:results-office31}
% \vspace*{-15pt}
% \end{table*}




 \begin{table*}[htbp]
    \centering
    \resizebox{0.7\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Method & A$\rightarrow$W & D$\rightarrow$W & W$\rightarrow$D & A$\rightarrow$D & D$\rightarrow$A & W$\rightarrow$A & Avg \\
\midrule
ResNet~\cite{he2016deep} & 68.4$\pm$0.2 & 96.7$\pm$0.1 & 99.3$\pm$0.1 & 68.9$\pm$0.2 & 62.5$\pm$0.3 & 60.7$\pm$0.3 & 76.1\\
DANN~\cite{ganin2016domain} & 82.0$\pm$0.4 & 96.9$\pm$0.2 & 99.1$\pm$0.1 & 79.7$\pm$0.4 & 68.2$\pm$0.4 & 67.4$\pm$0.5 & 82.2 \\
JAN~\cite{long2017deep} & 85.4$\pm$0.3 & 97.4$\pm$0.2 & 99.8$\pm$0.2 & 84.7$\pm$0.3 & 68.6$\pm$0.3 & 70.0$\pm$0.4 & 84.3 \\
GTA~\cite{sankaranarayanan2018generate} & 89.5$\pm$0.5 & 97.9$\pm$0.3 & 99.8$\pm$0.4 & 87.7$\pm$0.5 & 72.8$\pm$0.3 & 71.4$\pm$0.4 & 86.5 \\
MCD~\cite{saito2018maximum} & 88.6$\pm$0.2 & 98.5$\pm$0.1 & 100.0$\pm$.0 &92.2$\pm$0.2 & 69.5$\pm$0.1 & 69.7$\pm$0.3 & 86.5 \\
MDD~\cite{zhang2019bridging} & 94.5$\pm$0.3 & 98.4$\pm$0.1 & 100.0$\pm$.0 &93.5$\pm$0.2 &74.6$\pm$0.3& 72.2$\pm$0.1 & 88.9 \\
KL~\cite{nguyen2021kl} & 87.9$\pm$0.4 & 99.0$\pm$0.2 & 100.0$\pm$0.0 & 85.6$\pm$0.6 & 70.1$\pm$1.1 & 69.3$\pm$0.7 & 85.3 \\
CDAN~\cite{long2018conditional} & 94.1$\pm$0.1 & 98.6$\pm$0.1 & 100.0$\pm$.0 & 92.9$\pm$0.2 & 71.0$\pm$0.3 & 69.3$\pm$0.3 & 87.7 \\
f-DAL~\cite{acuna2021f} & \textbf{95.4}$\pm$0.7 & \textbf{98.8}$\pm$0.1 & \textbf{100.0}$\pm$.0 & 93.8$\pm$0.4 & 74.9$\pm$1.5 & 74.2 $\pm$0.5 & 89.5 \\
%f-DAL+Alignment~\cite{acuna2021f} & 93.4$\pm$0.4 & \textbf{99.0}$\pm$0.1 & \textbf{100.0}$\pm$.0 & 94.8$\pm$0.6 & 73.6$\pm$0.2 & 74.6$\pm$0.4 & 89.2 \\
\midrule
CS-adv (Ours) & 95.1$\pm$0.6 & \textbf{98.8}$\pm$0.1 &	99.7$\pm$0.1 & \textbf{94.0}$\pm$0.5 &	\textbf{76.2}$\pm$0.3 & \textbf{76.4}$\pm$0.4 &	\textbf{90.0} \\
\bottomrule
\end{tabular}%
}
\caption{Comparative results (Accuracy \%) of different methods on \textbf{Office-31}.}
\label{tab:results-office31}
\end{table*}

==> Tables/syn_mmd_cs.tex <==
% \begin{table}[h]
% \centering
% \begin{tabular}{lcccccc}
% \toprule
%  & \multicolumn{3}{c}{Conditional CS} & \multicolumn{3}{c}{Conditional MMD} \\
% \cmidrule(r){2-4} \cmidrule(r){5-7}
%  & (a) & (b) & (c) & (a) & (b) & (c) \\
% \midrule
% (a) & 0.05 & 1 & 1 & 0.06 & 0 & 0 \\
% (b) & 1 & 0.08 & 0.92 & 0 & 0.04 & 0 \\
% (c) & 1 & 0.91 & 0.10 & 0 & 0 & 0.10 \\
% \bottomrule
% \end{tabular}
% \caption{Power test for conditional CS and conditional MMD. An idea result is a full-one matrix with 0 on the diagonal.}
% \label{tab:syn_mmd_cs}
% \end{table}

\begin{wraptable}{r}{0.5\textwidth}  % "r" for right alignment and width of the table
\centering
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Conditional CS} & \multicolumn{3}{c}{Conditional MMD} \\
\cmidrule(r){2-4} \cmidrule(r){5-7}
 & (a) & (b) & (c) & (a) & (b) & (c) \\
\midrule
(a) & 0.05 & 1 & 1 & 0.06 & 0 & 0 \\
(b) & 1 & 0.08 & 0.92 & 0 & 0.04 & 0 \\
(c) & 1 & 0.91 & 0.10 & 0 & 0 & 0.10 \\
\bottomrule
\end{tabular}
\caption{Power test for conditional CS and conditional MMD. An ideal result is a full-one matrix with 0 on the diagonal.}
\label{tab:syn_mmd_cs}
\end{wraptable}

% \begin{table}[htbp]
%     \begin{minipage}[b]{0.3\textwidth}   
%         \centering 
%         \scalebox{0.6}{
%         \begin{tabular}{lcccccc}
%         \toprule
%          & \multicolumn{3}{c}{Conditional CS} & \multicolumn{3}{c}{Conditional MMD} \\
%         \cmidrule(r){2-4} \cmidrule(r){5-7}
%          & (a) & (b) & (c) & (a) & (b) & (c) \\
%         \midrule
%         (a) & 0.05 & 1 & 1 & 0.06 & 0 & 0 \\
%         (b) & 1 & 0.08 & 0.92 & 0 & 0.04 & 0 \\
%         (c) & 1 & 0.91 & 0.10 & 0 & 0 & 0.10 \\
%         \bottomrule
%         \end{tabular}}
%         \caption{Caption for table}
%         \label{tab:table}
%     \end{minipage}
% \end{table}



% \begin{figure}[htbp]
%     \begin{minipage}[b]{0.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Figures/power_mean.pdf}
%         \caption{Caption for image 1}
%         \label{fig:image1}
%         \vspace{1cm} % Adjust as needed
%         \includegraphics[width=\linewidth]{Figures/power_variance.pdf}
%         \caption{Caption for image 2}
%         \label{fig:image2}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.45\linewidth}
%         \centering
%         \begin{tabular}{lcccccc}
%         \toprule
%         & \multicolumn{3}{c}{Conditional CS} & \multicolumn{3}{c}{Conditional MMD} \\
%         \cmidrule(r){2-4} \cmidrule(r){5-7}
%         & (a) & (b) & (c) & (a) & (b) & (c) \\
%         \midrule
%         (a) & 0.05 & 1 & 1 & 0.06 & 0 & 0 \\
%         (b) & 1 & 0.08 & 0.92 & 0 & 0.04 & 0 \\
%         (c) & 1 & 0.91 & 0.10 & 0 & 0 & 0.10 \\
%         \bottomrule
%         \end{tabular}
%         \caption{Comparison of Conditional CS and Conditional MMD}
%         \label{tab:comparison}
%     \end{minipage}
% \end{figure}



